Mass Gatherings for Political Expression Had No Discernable Association with the Local Course of the COVID-19 Pandemic in the USA in 2020 and 2021

Epidemic disease can spread during mass gatherings. We assessed the impact on the local-area trajectory of the COVID-19 epidemic of a type of mass gathering about which comprehensive data were available. Here, we examined five types of political events in 2020 and 2021: the US primary elections; the US Senate special election in Georgia; the gubernatorial elections in New Jersey and Virginia; Donald Trump's political rallies; and the Black Lives Matter protests. Our study period encompassed over 700 such mass gatherings during multiple phases of the pandemic. We used data from the 48 contiguous states, representing 3,119 counties, and we implemented a novel extension of a recently developed non-parametric, generalized difference-in-difference estimator with a (high-quality) matching procedure for panel data to estimate the average effect of the gatherings on local mortality and other outcomes. There were no statistically significant increases in cases, deaths, or a measure of epidemic transmissibility (Rt) in a 40-day period following large-scale political activities. We estimated small and statistically insignificant effects, corresponding to an average difference of -0.0567 deaths (95% CI = -0.319, 0.162), and 8.275 cases (95% CI = -1.383, 20.7), on each day, for counties that held mass gatherings for political expression compared to matched control counties. In sum, there is no statistical evidence of a material increase in local COVID-19 deaths, cases, or transmissibility after mass gatherings for political expression during the first two years of the pandemic in the USA. This may relate to the specific manner in which such activities are typically conducted.

==> preamble.tex <==
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\renewcommand\footnote[1]{}
